Instrumental performance and results from testing of the BLAST-TNG receiver, submillimeter optics, and MKID arrays

Polarized thermal emission from interstellar dust grains can be used to map magnetic fields in star forming molecular clouds and the diffuse interstellar medium (ISM). The Balloon-borne Large Aperture Submillimeter Telescope for Polarimetry (BLASTPol) flew from Antarctica in 2010 and 2012 and produced degree-scale polarization maps of several nearby molecular clouds with arcminute resolution. The success of BLASTPol has motivated a next-generation instrument, BLAST-TNG, which will use more than 3000 linear polarization sensitive microwave kinetic inductance detectors (MKIDs) combined with a 2.5m diameter carbon fiber primary mirror to make diffraction-limited observations at 250, 350, and 500 $\mu$m. With 16 times the mapping speed of BLASTPol, sub-arcminute resolution, and a longer flight time, BLAST-TNG will be able to examine nearby molecular clouds and the diffuse galactic dust polarization spectrum in unprecedented detail. The 250 $\mu$m detector array has been integrated into the new cryogenic receiver, and is undergoing testing to establish the optical and polarization characteristics of the instrument. BLAST-TNG will demonstrate the effectiveness of kilo-pixel MKID arrays for applications in submillimeter astronomy. BLAST-TNG is scheduled to fly from Antarctica in December 2017 for 28 days and will be the first balloon-borne telescope to offer a quarter of the flight for "shared risk" observing by the community.

==> tab_loading.tex <==
\begin{table}[t]

%\singlespace
%\footnotesize
%\rotate
%\tabletypesize{\footnotesize}
%\tableheadfrac{}
\newcommand\T{\rule{0pt}{3ex}}       % Top strut
\newcommand\B{\rule[-2ex]{0pt}{0pt}} % Bottom strut
\vspace{3 mm}
\begin{center}
\caption{Table of 4\,K loading values and resultant hold times \label{tab:loading}}
\vspace{3 mm}
\renewcommand{\arraystretch}{1.2}%
\begin{tabular}{cccc}
\hline
\hline
\T He Gas Flow(mm) & He Gas Flow(L/mi) & 4\,K Loading P(mW) & Hold Time (Days) \B \\
\hline
\T 40 & 2.30 & 131 & 58\\
50 & 3.15 & 180 & 42\\
60 & 3.98 & 228 & 33\\
70 & 4.78 & 273 & 28\\
80 & 5.54 & 317 & 24\\
90 & 6.27 & 359 & 21\\
100 & 6.99 & 399 & 19\\
&&&\B \\                                                    
\hline
\end{tabular}
\end{center}
%\tablenotetext{a}{}
%\tablecomment{}
\end{table}


